A Unified Off-Policy Evaluation Approach for General Value Function

General Value Function (GVF) is a powerful tool to represent both the {\em predictive} and {\em retrospective} knowledge in reinforcement learning (RL). In practice, often multiple interrelated GVFs need to be evaluated jointly with pre-collected off-policy samples. In the literature, the gradient temporal difference (GTD) learning method has been adopted to evaluate GVFs in the off-policy setting, but such an approach may suffer from a large estimation error even if the function approximation class is sufficiently expressive. Moreover, none of the previous work have formally established the convergence guarantee to the ground truth GVFs under the function approximation settings. In this paper, we address both issues through the lens of a class of GVFs with causal filtering, which cover a wide range of RL applications such as reward variance, value gradient, cost in anomaly detection, stationary distribution gradient, etc. We propose a new algorithm called GenTD for off-policy GVFs evaluation and show that GenTD learns multiple interrelated multi-dimensional GVFs as efficiently as a single canonical scalar value function. We further show that unlike GTD, the learned GVFs by GenTD are guaranteed to converge to the ground truth GVFs as long as the function approximation power is sufficiently large. To our best knowledge, GenTD is the first off-policy GVF evaluation algorithm that has global optimality guarantee.

==> application.tex <==
\section{Examples of Forward and Backward GVFs}\label{sc: application}
In this section, we present a number of example forward and backward GVFs in RL applications.
\subsection{Example Forward GVFs}
The forward GVF in \Cref{def:forwardGVF} arises naturally in the following RL applications. 

{\bf Case I: Variance of Reward-To-Go. } In risk-sensitive domains such as finance, process control and clinical decision making \cite{sharpe1966mutual,mannor2013algorithmic,tamar2013variance,tamar2012policy,ruszczynski2010risk,sato2001td,sobel1982variance,jain2021variance}, in addition to the mean $J_\pi$ of the "reward-to-go", we are also interested in the variance of $J_\pi$ \cite{sharpe1966mutual,shortreed2011informing}, which is given by $\text{Var}[J_\pi|(s_0,a_0)=(s,a)]= H_\pi(s,a) - Q^2_\pi(s,a)$, where $H_\pi$ is the second moment of $J_\pi$, i.e., $H_\pi(s,a)=\mE[J_\pi^2|(s_0,a_0)=(s,a),\pi]$. \cite{tamar2016learning} shows that $H_\pi$ satisfies
\begin{flalign}
H_\pi = R^2 + 2\gamma M_R \msP_\pi Q_\pi + \gamma^2 \msP_\pi H_\pi,\label{eq: 32}
\end{flalign}
where $M_R = \diag(R)\in\mR^{|\mcs||\mca|\times |\mcs||\mca|}$. \Cref{eq: 32} implies that $H_\pi$ is the mean of the accumulation of signal $C(s,a)=r(s,a)^2 + 2\gamma \mE[Q_\pi(s^\prime,a^\prime)|s,a]$ with discounted factor $\gamma^2$. Since $C(s,a)$ is a function of the reward $r(s,a)$ and value function $Q_\pi(s,a)$, we consider the joint vector of $Q_\pi$ and $H_\pi$ as $G_\pi$, i.e., $G_\pi = [Q^\top_\pi, H^\top_\pi]^\top$. We have that $G_\pi$ satisfies the general Bellman equation in \cref{forward_GBE} with $B$ and $M_\pi$ specified as
\begin{flalign}\label{eq: variance}
B = \left[\begin{array}{c}
R\\
R^2
\end{array}
\right],\quad
M_\pi = \left[\begin{array}{cc}
\gamma\msP_\pi & 0 \\
2\gamma M_R\msP_\pi & \gamma^2 \msP_\pi
\end{array}
\right].
\end{flalign}
We consider the setting in which reward is bounded, i.e., $r(s,a)\leq C_R$ for all $(s,a)\in\mcs\times\mca$. 
%The following lemma establishes the contraction property of $T_{G,\pi}$ in this case.
%\begin{lemma}\label{lemma: contraction_variance}
% Consider $T_{G,\pi}$ in \cref{forward_GBE} with $R_\pi$ and $M_\pi$ specified in \cref{eq: variance}. For any vector $v = [\Delta_Q^\top, \Delta_H^\top]^\top\in\mR^{2|\mcs||\mca|\times 1}$, in which $\Delta_Q, \Delta_H\in\mR^{|\mcs||\mca|\times 1}$, we define the norm $\lalpha{\cdot}$ as $\lalpha{v} = \alpha_G \lsmu{\Delta_Q} + (1-\alpha_G)\lsmu{\Delta_H}$, where $\alpha_G = \frac{4\gamma C_R}{1-\gamma + 4\gamma C_R}$. We have $T_{G,\pi}$ is $(\frac{1+\gamma}{2})$--contraction in $\lalpha{\cdot}$--norm.
%\end{lemma}

{\bf Case II: Gradient of Q-function.} Suppose that the policy is parametrized by a smooth function $\pi_w$, in which $w\in\mR^{d_w}$ is the parameter. Then the gradient $\nabla_w Q_{\pi}(s,a)$ of the Q-function w.r.t $w$ plays an important role in several RL applications such as variance reduced policy gradient \cite{huang2020importance} and on- and off-policy policy optimization \cite{xu2021doubly,silver2014deterministic,kallus2020statistically,comanici2018knowledge}. Specifically, \cite{xu2021doubly,kallus2020statistically,comanici2018knowledge} shows that $\nabla_wQ_\pi$ satisfies:
%the following equation
\begin{flalign}
\nabla_w Q_{\pi} = \gamma [\msP_\pi\otimes \msI_{d_w}] [\nabla_w{\rm\Pi}_{\pi_w}\cdot Q_{\pi}] + \gamma [\msP_\pi \otimes \msI_{d_w}]\nabla_wQ_{\pi},\label{eq: 33}
\end{flalign}
where $\nabla_w{\rm\Pi}_{\pi_w}\in\mR^{d_w|\mcs||\mca|}$ is obtained by stacking $\nabla_w\log(\pi(s,a))$ over $\mcs\times\mca$, i.e., $[\nabla_w{\rm\Pi}_{\pi_w}](s,a)=\nabla_w\log(\pi_w(s,a))$, and $[\nabla_w{\rm\Pi}_{\pi_w}\cdot Q_{\pi}]\in\mR^{d_w|\mcs||\mca|}$ is  element-wise product between $\nabla_w{\rm\Pi}_{\pi_w}$ and $Q_\pi$, i.e., $[\nabla_w{\rm\Pi}_{\pi_w}\cdot Q_{\pi}](s,a)=\nabla_w\log(\pi_w(s,a))Q_{\pi}(s,a)$. \Cref{eq: 33} implies that $\nabla_wQ_\pi$ is the mean of the accumulation of signal $C(s,a)=\gamma \mE[Q_\pi(s^\prime,a^\prime)\nabla_w\log(\pi_w(s^\prime,a^\prime))|s,a]$ with the discounted factor $\gamma$. Let $G_\pi = [Q^\top_\pi, \nabla_wQ^\top]^\top$. We have that $G_\pi$ satisfies the general Bellman equation in \cref{forward_GBE} with $B$ and $M_\pi$ specified as
\begin{flalign}\label{eq: dq}
B = \left[\begin{array}{c}
R\\
0
\end{array}
\right],\quad
M_\pi = \left[\begin{array}{cc}
\gamma\msP_\pi & 0 \\
\gamma[\msP_\pi\otimes \msI_{d_w}] \diag(\nabla_w{\rpii}_{\pi_w}) & \gamma\msP_\pi\otimes\msI_{d_w}
\end{array}
\right],
\end{flalign}
where $\diag(\nabla_w{\rpii}_{\pi_w}) \in\mR^{d_w|\mcs||\mca|\times |\mcs||\mca|}$ is obtained by arranging $\nabla_w\log(\pi(s,a))\in\mR^{d_w}$ diagonally. Without loss of generality, we assume that the score function is bounded \cite{sutton2018reinforcement,sutton2000policy,xu2020improving}, i.e., $\ltwo{\nabla_w\log(\pi_w(s,a))}\leq C_{\rm\Pi}$ for all $(s,a)\in\mcs\times\mca$. 
%We provide the following lemma to characterize the contraction property of $T_{G,\pi}$ in this problem.
%\begin{lemma}\label{lemma: derivative_q}
%	Consider $T_{G,\pi}$ in \cref{forward_GBE} with $R_\pi$ and $M_\pi$ specified in \cref{eq: dq}. For any vector $v = [\Delta_Q^\top, \Delta_{dQ}^\top]^\top\in\mR^{(1+d_w)|\mcs||\mca|\times 1}$, in which $\Delta_Q\in\mR^{|\mcs||\mca|\times 1}$ and $\Delta_{dQ}\in\mR^{d_w|\mcs||\mca|\times 1}$, we define the norm $\lalpha{\cdot}$ as $\lalpha{v} = \alpha_G \lsmu{\Delta_Q} + (1-\alpha_G)\lsmu{\Delta_{dQ}}$, where $\alpha_G = \frac{2\gamma C_{\rpii}}{1-\gamma + 2\gamma C_{\rpii}}$. We have $T_{G,\pi}$ is $(\frac{1+\gamma}{2})$--contraction in $\lalpha{\cdot}$--norm.
%\end{lemma}

{\bf Case III: Stochastic Value Gradient.} The stochastic value gradient (SVG) method combines advantages of model-based and model-free methods, in which both the estimated model and value function are updated to evaluate the policy gradient \cite{heess2015learning}. In the framework of SVG, the reward $r(s,a)$ is differentiable with respect to both $s\in\mR^{d_s}$ an $a\in\mR^{d_a}$, the stochastic policy takes the form $a=\pi(s,w)+\eta$, and the transition probability is modelled as $s^\prime = f(s,a)+\xi$, where $\pi: \mcs\rightarrow \mca$ and $f: \mcs\times\mca\rightarrow \mcs$ are deterministic mappings, $w\in\mR^{d_w}$ is the policy parameter, and $\eta\sim P(\eta)$ and $\xi\sim P(\xi)$ are noise variables. We abbreviate the partial differentiation using subscripts as $g_x\triangleq \partial g/\partial x$. The gradient of the $Q$-function w.r.t the policy parameter $w$ is given by \cite{heess2015learning}
\begin{flalign}
Q_s &= (R_s + {\rm\Pi}_s R_a) + \gamma ({\rm\Pi}_s F_a + F_s)([\msP_\pi\otimes \msI_{d_s}] Q_s),\nonumber\\
Q_a &= R_a + \gamma F_a [\msP_\pi\otimes \msI_{d_s}] Q_s + \gamma [\msP_\pi\otimes \msI_{d_a}]Q_a,\nonumber\\
\nabla_wQ_\pi &= {\rm \Pi}_w Q_a + \gamma [\msP_\pi\otimes \msI_{d_w}]\nabla_wQ_\pi,\label{eq: 41}
\end{flalign}
where $R_s\in\mR^{d_s|\mcs||\mca|}$ and $R_a \in\mR^{d_a|\mcs||\mca|}$ are vectors obtained via stacking partial derivatives $r_s(s,a) \in\mR^{d_s}$ and $r_a(s,a)\in\mR^{d_a}$ over $(s,a)\in\mcs\times\mca$, and ${\rm\Pi}_s=\diag(\pi_s)\in \mR^{d_s|\mcs||\mca|\times d_a|\mcs||\mca|}$, ${\rm\Pi}_w=\diag(\pi_w)\in \mR^{d_w|\mcs||\mca|\times d_a|\mcs||\mca|}$, $F_s=\diag(f_s)\in \mR^{d_s|\mcs||\mca|\times d_s|\mcs||\mca|}$, and $F_a=\diag(f_a)\in \mR^{d_a|\mcs||\mca|\times d_s|\mcs||\mca|}$ are Jacobian matrices. 
%Specifically, $Q_s$ can be viewed as accumulation of signal $C_1(s,a) = r_s(s,a) + \pi_s(s,a)r_a(s,a)$ with discounted matrix $\gamma_1(s,a)=\gamma(\pi_s(s,a)f_a(s,a)+f_s(s,a))$, $Q_a$ as accumulation of signals $C_2(s,a)=r_a(s,a) + \gamma f_a(s,a)\mE[Q_s(s^\prime,a^\prime)|s,a]$ with discounted factor $\gamma_2(s,a)=\gamma$, and $\nabla_wQ_\pi$ as accumulation of $C_3(s,a)=\pi_w(s,a)Q_a(s,a)$ with discounted factor $\gamma_3(s,a)=\gamma$, respectively. 
Consider GVF defined as $G_\pi=[Q^\top_s, Q^\top_a, \nabla_wQ^\top_\pi]^\top$. Then $G_\pi$ satisfies the general Bellman equation in \cref{forward_GBE} with $B$ and $M_\pi$ specified by
\begin{flalign}
B &= \left[\begin{array}{c}
R_s + {\rm\Pi}_s R_a\\
R_a\\
{\rm\Pi}_w Q_a
\end{array}
\right],\quad
M_\pi = \left[\begin{array}{ccc}
\gamma({\rm\Pi}_s F_a + F_s)[\msP_\pi\otimes \msI_s] & 0 & 0  \\
\gamma F_a [\msP_\pi\otimes \msI_s] & \gamma[\msP_\pi\otimes \msI_a] &  0 \\
0 & {\rm\Pi}_w & \gamma [\msP_\pi\otimes \msI_{d_w}]
\end{array}
\right].\label{eq: svg}
\end{flalign}
We consider the setting in which $\lF{f_a(s,a)}\leq C_a$ and $\lF{\pi_w(s,a)}\leq C_w$ for all $(s,a)\in\mcs\times\mca$. To establish the contraction property of $G_\pi$, we make the following "non-expansive" assumption for the transition matrix $\gamma_1(s,a)=\gamma({\rm\Pi}_s F_a + F_s)$.
\begin{assumption}[Non-expansive]\label{ass9}
	For any $v\in\mR^{d_s\times 1}$, we have $\lmu{ ({\rm\Pi}_s F_a + F_s)v} \leq \lmu{v}$.
\end{assumption}
\Cref{ass9} is the minimum requirement to guarantee the value of $Q_s$ to be bounded. It can be satisfied by selecting appropriate policy class $\pi_w$ and model approximation $f$ together with the feature design of both state $s$ and action $a$. 

%{\bf Case IV: Option Learning.} In the option framework \cite{sutton1999between}, an option is defined as $(\pi_o,\lambda_o, \mco)$, where $\pi_o: \mcs\times\mca\rightarrow [0,1]$ is an intra-option policy, $\lambda_o: \mcs\rightarrow[0,1]$ is a termination function, and $\mco$ is the option set. In this framework, the policy $\pi$ is defined over the option-state space, i.e., $\pi: \mco\times\mcs \rightarrow[0,1]$. At time step $t$, an agent at state $s_t$ either terminates the previous option $o_{t-1}$ with probability $\lambda_{o_{t-1}}(s_t)$ and initiates a new option $o_t$ according to policy $\pi(\cdot|s_t)$, or proceeds with the previous option $o_{t-1}$ with probability $1-\lambda_{o_{t-1}}(s_t)$ and sets $o_t = o_{t-1}$. Then an action $a_t$ is selected according to $\pi_{o_t}(\cdot|s_t)$. The agent receive a reward $r(s_t,a_t)$. Similar to regular MDP, here we define state-option value function as $Q_\pi(s,o)=\int_{a}\pi(a|s)Q_\pi(s,o,a)da$, where $Q_\pi(s,o,a)=\mE[\sum_{t=0}^{\infty}\gamma^t r(s_t,a_t)|s_0=s,a_0=a,o_0 = o]$. We consider evaluate the state-option value function $Q_\pi(s,o)$. \cite{zhang2019dac} shows that 
%\begin{flalign}\label{eq: 40}
%Q^\mco_\pi = R + \gamma P^{\lambda,\mco}_\pi Q^\mco_\pi,
%\end{flalign}
%where $[P^{\lambda,\mco}_\pi]((s,o),(s^\prime,o^\prime))=[(1-\lambda_o(s^\prime))\mathbb{1}_{o^\prime=o}+\lambda_o(s^\prime)\pi(o^\prime|s^\prime)]\msP(s^\prime|s,o)$, where $\msP(s^\prime|s,o)=\int_{a}\pi_o(a|s)\msP(s^\prime|s,a)$. Let $Y_\pi(x) = Q_\pi(s,o)$, $C(x_t)=r(s_t,a_t)$ and $m(x,x_{t+1})=\gamma$, it can be checked that $Y_\pi$ satisfies the general Bellman equation defined in \cref{eq: return}.

\subsection{Example Backward GVFs}
The backward GVF in \Cref{def:backwardGVF} also arises in the following important RL applications.

{\bf Case IV: Anomaly Detection.} \cite{zhang2020learning} has systemically discussed the application of retrospective knowledge in anomaly detection. Let $i(s,a)$ be the cost that an agent consumes when taking action $a$ at state $s$, and $e_\pi(s,a)$ be the cost that an agent is expected to consume given the current status when following a predefined policy $\pi$. If the actual cost of the agent deviates too much from $e_\pi$, the agent may likely experience anomalous events. For simplicity, we consider the setting when $\gamma(s,a)=\gamma$. It can be shown that $e_\pi$ satisfies the following equation
\begin{flalign}
e_\pi =   i +  \gamma U^{-1}_\pi \msP^\top_\pi U_\pi e_\pi.\label{eq: 34}
\end{flalign}
Clearly, \cref{eq: 34} satisfies the general backward Bellman equation in \cref{backward_GBE} by letting $B=i$, $M_\pi = \gamma\msP_\pi$, and $\hat{G}_\pi = e_\pi$. 
%The following lemma characterizes the contraction property of $\hat{T}_{G,\pi}$.
%\begin{lemma}\label{lemma: contraction_detection}
%	Consider $\hat{T}_{G,\pi}$ in \cref{backward_GBE} with $R_\pi = i$ and $M_\pi = \gamma\msP_\pi$. We have $\hat{T}_{G,\pi}$ is $\gamma$--contraction in $\lsmu{\cdot}$--norm.
%\end{lemma}


{\bf Case V: Gradient of Logarithmic Stationary Distributions.} In the policy parameterization setting, the gradient of logarithmic stationary distribution $\nabla_w \log(\mu_{\pi})(s,a)$ has been used in policy gradient estimation \cite{kallus2020statistically,xu2021doubly,morimura2010derivatives} and maximum entropy exploration \cite{hazan2019provably}. It has been shown in \cite{morimura2010derivatives,xu2021doubly} that $\nabla_w \log(\mu_{\pi})(s,a)$ satisfies the following equation
\begin{flalign}
{\rm\Psi}_\pi = \nabla_w{\rm\Pi}_{\pi_w} + U^{-1}_\pi[\msP_\pi^\top \otimes \msI_{d_w}] U_\pi{\rm\Psi}_\pi , \label{eq: 35}
\end{flalign}
where ${\rm\Psi}_\pi $ is obtained via stacking $\nabla_w\log(\mu_{\pi}(s,a))$ over $\mcs\times\mca$, i.e., $[{\rm\Psi}_\pi](s,a) = \nabla_w\log(\mu_{\pi_w}(s,a))$. Here, $\nabla_w\log\mu_\pi$ can be viewed as a backward accumulation of the signal $C(s,a)=\nabla_w \log(\pi(s,a))$ with the discounted factor $\gamma=1$. Define the backward GVF as $\hat{G}_\pi={\rm\Psi}_\pi$. It is clear that $\hat{G}_\pi$ satisfies the general backward Bellman equation in \cref{backward_GBE} with $B$ and $M_\pi$ specified by
\begin{flalign}\label{eq: 46}
B = \nabla_w{\rm\Pi}_{\pi_w},\qquad M_\pi = \msP_\pi^\top \otimes \msI_{d_w}.
\end{flalign}
%Note that $\hat{T}_{G,\pi}$ in this setting is not a contraction, i.e., the fixed point of $\hat{T}_{G,\pi}$ is not unique. To see this, define a feature matrix $E = [E_1, \cdots, E_{d_w}]\in\mR^{d_w|\mcs||\mca|\times d_w}$, in which $E_i=[e_i^\top, \cdots, e_i^\top]^\top\in\mR^{d_w|\mcs||\mca|\times 1}$ and $e_i\in \mR^{d_w\times 1}$ is an "one-hot" vector whose $i$-th component is $1$ and the rest are $0$. It can be checked that if ${\rm\Psi}_\pi$ is a fixed point of $\hat{T}_{G,\pi}$, i.e., ${\rm\Psi}_\pi = \hat{T}_{G,\pi}{\rm\Psi}_\pi$, then ${\rm\Psi}_\pi + E\xi$ is also a fixed point of $ \hat{T}_{G,\pi}$ for any $\xi\in\mR^{d_w\times 1}$. We define ${\rm\Psi}^*_\pi$ as a fixed point of $ \hat{T}_{G,\pi}$ which is orthogonal to the linear space spanned by the column of $E$ w.r.t. $\lsmu{\cdot}$--norm. In this problem, we only consider evaluating $G_\pi = {\rm\Psi}^*_\pi$, which is uniquely defined.

%In the averaged MDP setting, the value function is defined as the expected accumulation of the reward subtracted by the average of reward over the stationary distribution, i.e., $Q_\pi(s,a)=\mE[\sum_{t=0}^{\infty}r(s,a)-J(\pi)|(s_0,a_0)=(s,a),\pi]$, where $J(\pi)=\mE_{\mu_\pi}[r(s,a)]$. Readers may wonder why we do not adopt a similar formulation here. We provide the following lemma to show that there is no need to subtract an average of score function to define a GVF here, as the average of the score function over the stationary distribution is $0$.
%\begin{lemma}\label{lemma15}
%	For any ergodic MDP and differentiable policy $\pi_w$. We have $\mE_{\mu_\pi}[\nabla_w\log(\pi(s,a))]=0$.
%\end{lemma}

%However, as we will show in \Cref{sc: app_app}, with appropriately chosen base function ${\rm\Phi}$, we can show that the composite operator $\hat{T}_{G,\pi}{\rm\Gamma}_{\mu_\pi}$ is a contraction, where ${\rm\Gamma}_{\mu_{\pi}}$ is a projection operator that will be specified in the next section.



